A hierarchical Bayesian framework for cosmology using Type 1 AGN variability

Independent luminosity-distance probes beyond the Type Ia supernova range are needed to test cosmic expansion at high redshift. Type 1 AGN are abundant at \(z>2\), but their use for cosmology requires standardizable observables with controlled scatter, redshift dependence, and measurement uncertainty. We present a hierarchical Bayesian framework for cosmology using AGN variability, based on the empirical anti-correlation between optical/UV variability amplitude and luminosity. The method targets the moderate-baseline regime of current wide-field time-domain surveys, where individual light curves cannot typically identify the full long-timescale stochastic process, but can constrain finite-window brightness and short-lag variability. Each light curve is fitted independently to obtain posterior samples of these summaries, which are then importance-reweighted under a population model relating variability to luminosity, rest-frame wavelength, intrinsic scatter, and the assumed distance-redshift relation. This framework propagates object-level uncertainty while avoiding repeated light-curve likelihood evaluations during cosmological inference, making catalogue-scale analyses feasible. Using Gaia DR3-like G-band simulations matched to real Gaia cadences, noise properties, and quality cuts, we show that finite-baseline light curves are more robustly summarized by window-averaged brightness and short-lag variability than by the separate long-timescale parameters of stochastic models. End-to-end closure tests recover the injected variability-luminosity relation, intrinsic scatter, and distance-redshift parameters up to the expected calibration degeneracies. This Gaia G-band analysis establishes a proof of concept for AGN-variability distances in the moderate-baseline survey regime, with the main gains expected from Gaia DR4, ZTF, DESI-selected AGN samples, and Rubin/LSST-era data.

==> packages.tex <==
\RequirePackage{silence}
\WarningFilter{hyperref}{Option `pagecolor' is not available anymore}

\usepackage{jcappub} 
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{epigraph}
\setlength\epigraphrule{0pt}
\setlength\epigraphwidth{0.6\textwidth}
\usepackage{booktabs}

\usepackage{placeins}
\usepackage{soul}
\usepackage[normalem]{ulem}
\usepackage{float}
\usepackage{tabularx}
\usepackage{array}
\usepackage{ragged2e}
% \usepackage{txfonts}
% \usepackage{supertabular}
% \usepackage[math]{cellspace}
% \renewcommand{\cellspacetoplimit}{5pt}
% \renewcommand{\cellspacebottomlimit}{5pt}
\usepackage{xspace}
\usepackage[dvipsnames]{xcolor}

\definecolor{obsfill}{RGB}{235,235,235}
\definecolor{hyperfill}{RGB}{224,238,255}
\definecolor{s1blue}{RGB}{40,100,180}
\definecolor{s2orange}{RGB}{220,120,30}

\usepackage{fontawesome}
\usepackage{bm}
\usepackage{comment}
\usepackage{tikz}
\usetikzlibrary{
    arrows.meta,   
    positioning,   
    fit,           
    calc           
}

%\usepackage{hyperref}
%Not sure if these are allowed, but to keep the paragraph spacing looking ok.
%\setlength{\parindent}{0pt}
%\setlength{\parskip}{0.5em}

\newcommand{\maybeinclude}[3]{%
    \IfFileExists{#1}{%
        \begin{figure}[t]
            \centering
            \includegraphics[width=#2]{#1}
            \caption{#3}
        \end{figure}
    }{%
        \begin{figure}[t]
            \centering
            \fbox{\parbox{#2}{
                \textbf{Missing figure:} #1
            }}
            \caption{#3}
        \end{figure}
    }%
}
\hypersetup{
  colorlinks=true,
  allcolors=Blue,
  hypertexnames=false
}

% Journal macros used by ADS/NASA BibTeX entries
\providecommand{\aap}{Astron. Astrophys.}
\providecommand{\aj}{Astron. J.}
\providecommand{\apj}{Astrophys. J.}
\providecommand{\apjl}{Astrophys. J. Lett.}
\providecommand{\apjs}{Astrophys. J. Suppl.}
\providecommand{\jcap}{JCAP}
\providecommand{\mnras}{Mon. Not. Roy. Astron. Soc.}
\providecommand{\pasp}{Publ. Astron. Soc. Pac.}
\providecommand{\prd}{Phys. Rev. D}
\providecommand{\prl}{Phys. Rev. Lett.}

% commands
\newcommand{\lenstronomy}{\texttt{lenstronomy}\xspace}
\newcommand{\dolphin}{\texttt{dolphin}\xspace}
\newcommand{\amplification}{\bm{\mathcal{A}}}

\newcommand{\nlenses}{22\xspace}

% Roman subscripts and superscripts
\newcommand\e[1]{_{\mathrm{#1}}}
\newcommand\h[1]{^{\mathrm{#1}}}
\newcommand\U[1]{~\mathrm{#1}}


% Derivatives
\newcommand{\dd}{\mathrm{d}}
\newcommand{\Dd}{\mathrm{D}}
\newcommand{\pd}[3][]{\frac{\partial^{#1} #2}{\partial {#3}^{#1}}}
\newcommand{\ddf}[3][]{\frac{\dd^{#1} #2}{\dd {#3}^{#1}}}
\newcommand{\Ddf}[3][]{\frac{\Dd^{#1} #2}{\dd {#3}^{#1}}}
% comments
\newcommand{\nhc}[1]{{\color{ForestGreen} \texttt{[NH: #1]}}}
\newcommand{\nht}[1]{{\color{ForestGreen} {#1}}}
%\newcommand{\nht}[1]{{\color{black} {#1}}}

\newcommand{\DP}[1]{\textcolor{blue}{{\bf [DP: #1]}}}

\newcommand{\mwin}{m_{\rm win}}
\newcommand{\Dvar}{D}
\newcommand{\sigDRW}{\sigma_{\rm DRW}}
\newcommand{\tauDRW}{\tau_{\rm DRW}}


\providecolor{obsfill}{RGB}{220,220,220}
\definecolor{stageoneorange}{HTML}{00A6D6} % Stage 1: cyan
\definecolor{stagetwoblue}{HTML}{A51C5A}   % Stage 2: deep raspberry (so they are not the same as the ones for the different priors)
\providecolor{pgmfaint}{RGB}{210,210,210}

